Encapsulated generalized summation-by-parts formulations for curvilinear and non-conforming meshes

We extend the construction of so-called encapsulated global summation-by-parts operators to the general case of a mesh which is not boundary conforming. Owing to this development, energy stable discretizations of nonlinear and variable coefficient initial boundary value problems can be formulated in simple and straightforward ways using high-order accurate operators of generalized summation-by-parts type. Encapsulated features on a single computational block or element may include polynomial bases, tensor products as well as curvilinear coordinate transformations. Moreover, through the use of inner product preserving interpolation or projection, the global summation-by-parts property in extended to arbitrary multi-block or multi-element meshes with non-conforming nodal interfaces.

==> preamble.latex <==
% Number sets
\newcommand{\R}{{\mathbb R}}
\newcommand{\Z}{{\mathbb Z}}
\newcommand{\C}{{\mathbb C}}
\newcommand{\N}{{\mathbb N}}

% Brackets
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\snorm}[1]{\|#1\|^2}
\newcommand{\expect}[1]{\langle #1 \rangle}

% Paranthesis
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\lift}{\mathcal{L}}

% Math environments
\newtheorem{definition}{Definition}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}
\newtheorem{remark}{Remark}
%\newtheorem{proof}{Proof}


% Continuous variables
\newcommand{\var}{w}
\newcommand{\uv}{\vec{u}}
\newcommand{\It}{\tilde{I}}
\newcommand{\ins}{\mathcal{L}}
\newcommand{\itnorm}[1]{\| #1 \|_{\It}^2}

% Discrete variables
\newcommand{\bs}[1]{\boldsymbol{#1}}
\newcommand{\dvar}{\boldsymbol{W}}
\newcommand{\dins}{\boldsymbol{\ins}}
\newcommand{\uu}{\boldsymbol{u}}
\newcommand{\uunL}{\boldsymbol{u_{L,n}}}
\newcommand{\uutL}{\boldsymbol{u_{L,t}}}
\newcommand{\uunR}{\boldsymbol{u_{R,n}}}
\newcommand{\uutR}{\boldsymbol{u_{R,t}}}
\newcommand{\vv}{\boldsymbol{v}}
\newcommand{\pp}{\boldsymbol{p}}
\newcommand{\Dy}{\mathcal{D}_y}
\newcommand{\DDy}{\bm{\Dy}}
\newcommand{\Dx}{\mathcal{D}_x}
\newcommand{\DDx}{\bs{\Dx}}
\newcommand{\DnL}{\mathcal{D}_{L,n}}
\newcommand{\DnR}{\mathcal{D}_{R,n}}
\newcommand{\PP}{\bs{\mathcal{P}}}
\newcommand{\IIt}{\boldsymbol{\It}}

